Are Human-generated Demonstrations Necessary for In-context Learning?

Despite the promising few-shot ability of large language models (LLMs), the standard paradigm of In-context Learning (ICL) suffers the disadvantages of susceptibility to selected demonstrations and the intricacy to generate these demonstrations. In this paper, we raise the fundamental question that whether human-generated demonstrations are necessary for ICL. To answer this question, we propose self-contemplation prompting strategy (SEC), a paradigm free from human-crafted demonstrations. The key point of SEC is that, instead of using hand-crafted examples as demonstrations in ICL, SEC asks LLMs to first create demonstrations on their own, based on which the final output is generated. SEC is a flexible framework and can be adapted to both the vanilla ICL and the chain-of-thought (CoT), but with greater ease: as the manual-generation process of both examples and rationale can be saved. Extensive experiments in arithmetic reasoning, commonsense reasoning, multi-task language understanding, and code generation benchmarks, show that SEC, which does not require hand-crafted demonstrations, significantly outperforms the zero-shot learning strategy, and achieves comparable results to ICL with hand-crafted demonstrations. This demonstrates that, for many tasks, contemporary LLMs possess a sufficient level of competence to exclusively depend on their own capacity for decision making, removing the need for external training data. Code is available at https://github.com/ruili33/SEC.

==> asset/intro.tex <==
%图要不要一定放在第一页，图能不能放在摘要前面
\begin{figure}[!h]
    \vspace{-35pt}
    \centering
    \includegraphics[width=1.0\linewidth]{asset/prompt_examp.pdf}
    \caption{Comparison between Vanilla Few-shot Prompting and Self-Constructed Few-shot Prompting. Different parts of the prompt and results are highlighted with different colors for emphasis. }
    \label{fig:prompt}
    \vspace{-10pt}
\end{figure}
\section{Introduction}
\label{section:intro}
After extensive upscaling, Large Language Models (LLMs) \citep{openai2023gpt4,brown2020language,touvron2023llama,
zeng2022glm130b,chowdhery2022palm} exhibit a notable capability across an array of downstream NLP tasks. The paradigm of in-context learning (ICL), or known as few-shot learning (Figure \ref{fig:prompt} (b)), has been instrumental in the success of LLMs. With several annotated examples, LLMs witness a marked performance augmentation across myriad tasks.
%这里可以这么写吗？
chain-of-thought (CoT) Prompting \citep{wei2022chain}  further enhances the performance on reasoning-intensive tasks (the pink part in Figure \ref{fig:cot_prompt}).

% Acquire knowledge through analogy is the fundamental idea behind in-context learning\citep{dong2022survey}.  In few-shot learning, LLMs are given a handful of labelled examples along with the test sample (see the lower part of Figure \ref{fig:prompt}), commomly known as prompts or demonstrations, which acts as a reference for models to generalize to new tasks. Different from training or finetuning \citep{devlin-etal-2019-bert}, as a gradient free method in-context learning  enables the model to  optimize in a single API call. Considering the high cost and extensive computational resources required to finetune a LLM, in-context learning has gained increasing attention among the community with it's flexibility and capability.

% Nevertheless, prompting only with labelled training examples (aka. answer only prompting) still struggles on tasks involving multi-step reasoning. To enhance the performance on reasoning-intensive tasks,  Few-shot chain-of-thought (CoT) Prompting \citep{wei2022chain} incorporates step by step reasoning process into the prompt for LLMs, which is illustrated in the orange part in Figure \ref{fig:prompt}. On the other side, Zero-shot CoT \citep{kojima2022large}leverages a simple instruction in the prompt to elicit LLMs to think step by step. Usually, Zero-shot CoT performs slightly worse than Few-shot CoT, which aligns with intuition.
% As an emergent ability, CoT dramatically augments complex reasoning ability in sufficiently large-scale models.

Although ICL yields excellent performances, 
% it requires human-crafted  training examples and carefully designed rationales, 
% For example, for MMLU  \citep{hendrycksmeasuring}, a  multi-task language understanding benchmark with 52 different tasks, we need to meticulously construct 52 different set of prompts. 
% which is unavailable in many tasks. 
its inherent reliance on human-engineered training exemplars and rationales poses a significant constraint, particularly in tasks where such resources are scant.
Besides, the performance is susceptible to small perturbations in the prompt,
bringing high variance to the overall performance \citep{liu2022makes,lu2023dynamic,zhao2021calibrate}.  

Given these challenges, \citet{li2022self} proposed Self-Prompting framework, an automatic framework in Open-Domain Question Answering free from training datasets. It first queries LLMs for several rounds to generate a pseudo QA pair, which is subsequently reiterated to produce a pseudo QA dataset.  During the inference phase, it utilize a clustering-based retrieval strategy to select pertinent few-shot examples. However, the scope of the Self-Prompting framework remains circumscribed predominantly to ODQA, rendering its extrapolation to alternative domains challenging.
In CoT Prompting, Auto-CoT \citep{zhang2022automatic}  utilizes Zero-shot CoT \citep{kojima2022large} to generate the rationales.
%  for each training example previously sampled by clustering. 
However, Auto-CoT still relies on a training set. 
 Besides, these two mothods both involve querying the model multiple times and additional clustering, making them difficult to adopt in real applications.

To tackle these problems, we propose Self-Constructed Prompting, a prompting strategy that  works well
in few-shot (Self-Constructed Few-shot Prompting, shown in Figure \ref{fig:prompt}) and CoT scenarios (Self-Constructed CoT Prompting, shown in Figure \ref{fig:cot_prompt}). \footnote[1]{The prompts for all experiments are shown in Appendix \ref{section:app_det_prompt}. To enhance comprehension, we have simplified the presentation of Self-Constructed Prompting in the two figures. The original, unsimplified version is shown in Figure \ref{fig:fews_un} and Figure \ref{fig:cot_un} for reference. } 
% Examples of Self-Constructed Few-shot Prompting and Self-Constructed CoT Prompting are shown in Figure \ref{fig:prompt} and Figure \ref{fig:cot_prompt} respectively.


Taking Self-Constructed Few-shot Prompting as an example, it can be divided into two steps: Few-shot Example Generation and Vanilla Few-shot Prompting. In Few-shot Example Generation, we prompt LLMs to synthesize several few-shot examples only conditioned on the question of each test case. Then, we perform answer cleaning and few-shot extraction to the output to ensure the conformity of generared few-shot examples to our pre-established format criteria. Then, a concatenation of these few-shot examples with the test query ensues, adhering to the protocols of Vanilla Few-shot Prompting. 
For Self-Constructed CoT Prompting, we follow \citet{kojima2022large} and add instructions to explicitly instruct the model to generate the reasoning process along with each few-shot examples. 
% And we subsequently prompt the model using Vanilla CoT Prompting

% //////
Our study includes empirical evaluations spanning diverse domains, encompassing arithmetic reasoning, commonsense reasoning, multi-task language understanding, and code generation benchmarks. 
% We conducted our main experiments on ChatGPT (gpt-3.5-turbo), and we also provide insights into the effect of model size in the ablation study.
 With no access to training dataset or any human intervention, Self-Constructed  Prompting achieves comparable results to Vanilla Prompting across all benchmarks in both few-shot and CoT scenarios, including GSM8K (77.0\% vs 77.4\%) 
\citep{cobbe2021training}, MATH (33.5\% vs 31.2\%) \citep{hendrycks2021measuring}, MMLU (71.4 \% vs 70.4 \%) \citep{hendrycksmeasuring} and HumanEval (76.2 \% vs 73.2 \%) \citep{chen2021evaluating}.  This result suggests that LLMs harbor the potential  to reach the performance benchmarks set by Vanilla Prompting. Our other ablation experiments further provide nuanced insights into the relative proficiencies of Self-Constructed Prompting vis-à-vis Vanilla, as well as some angles for further refining and optimizing Self-Constructed Prompting.

As a new paradigm of prompting, Self-Constructed Prompting provides a more stable and comprehensible evaluation framework, for its non-reliance on human-mediated interventions or the necessity for labeled datasets.
Compared to previous automatic prompting methodologies, Self-Constructed Prompting totally relies on a single query to generate the few-shot examples. Its inherent simplicity, adaptability, and cost-efficiency make it easier to be widely adopted in practice.
Furthermore, Self-Constructed Prompting is an emergent ability, and the few-shot examples generated by LLMs exhibit completely different characteristics comparable to human-generated few-shot examples.



==> common_code.tex <==
\section{Commonsense Reasoning, Multi-task Language Understanding And Code Generation}
\subsection{Main results}
\begin{table}[htbp]

    \begin{tabular}[]{>{\centering\arraybackslash}p{4.04cm} | >{\centering\arraybackslash}p{2.0cm}>{\centering\arraybackslash}p{2.2cm}>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{1.6cm}}
    \toprule
     & ARC & MMLU & C-Eval &HumanEval \\
     \midrule
     Standard Few-shot        & 86.5\%          &70.4\%         &\textbf{55.0\%}    &\%\\
     Standard CoT             &\textbf{87.9\%}  &69.6\%         &53.1\%             &\%\\
     Self-Constructed Few-shot&85.9\%           &68.3\%         &54.0\%             &76.2\%\\
     Self-Constructed CoT     & 86.9\%          &\textbf{71.4\%}&54.6\%             &- \\
     Standard Few-shot        & 85.2\%          &70.0\%         &-~~(51.0\%)        &-~~(48.1\%)\\
     Published Results        &\scriptsize{25-shot\citep{openai2023gpt4}}&\scriptsize{5-shot\citep{openai2023gpt4}}&\scriptsize{0-shot\citep{huang2023c}}&\scriptsize{0-shot\citep{openai2023gpt4}}\\
     Standard CoT             & -               &67.3\%         & 54.6\%            &- \\
     Published Results        &                 &\scriptsize{5-shot\citep{fu2023chain}}&\scriptsize{5-shot\citep{huang2023c}}&\\
    %  \\
    \bottomrule
\end{tabular}
\caption{}
\label{table:other_main_results}
\end{table}

==> math.tex <==
\section{Arithmetic Reasoning}
\subsection{Main results}
%表格宽度可以再调整，节省一行
\begin{table}[htbp]

    \begin{tabular}[]{>{\centering\arraybackslash}p{4.04cm} | >{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{2.2cm}>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{2.6cm}}
    \toprule
     & MATH & GSM8K & MMLU Math &C-Eval STEM \\
     \midrule
     Standard Few-shot        & 20.3\%          &57.1\%         &45.1\%             &\textbf{53.2\%}\\
     Standard CoT             & 31.2\%          &74.3\%         &\textbf{58.3\%}    &50.5\%\\
     Self-Constructed Few-shot&18.1\%           &63.9\%         &45.9\%             &52.3\%\\
     Self-Constructed CoT     & \textbf{33.5\%} &\textbf{76.3\%}&56.6\%             &51.8\%\\
     Standard Few-shot        & -               &57.1\%         & -                 &-~~(49.0\%)\\
     Published Results        &                 &\scriptsize{5-shot\citep{openai2023gpt4}}&&\scriptsize{0-shot\citep{huang2023c}}\\
     Standard CoT             & -               &74.9\%         & 51.1\%            &52.9\%\\
     Published Results                  &&\scriptsize{8-shot\citep{fu2023chain}}&\scriptsize{5-shot\citep{fu2023chain}}&\scriptsize{5-shot\citep{huang2023c}}\\
    %  \\
    \bottomrule
\end{tabular}
\caption{Comparison between Self-Constructed  Prompting and Standard  Prompting in both CoT and answer only scenario.  All of the results including the published results are the performance of gpt-3.5-turbo model. Since the output limit of gpt-3.5-turbo model, we can only generate a limited amount of shots, so we run the Standard Few-shot Prompting and Standard CoT Prompting in the same number of shots to ensure a fair compete. The results of our experiments on Standard Few-shot Prompting and Standard CoT Prompting are presented in the rows     Standard Few-shot and Standard CoT in the table.}

%detailed to in the appendix
\label{table:math_main_results}
\end{table}
% \begin{wrapfigure}[15]{r}{0.48\textwidth}
%       \begin{center}
%         \includegraphics[width=0.45\textwidth]{asset/math_sub.pdf}
%       \end{center}
%       \captionsetup{skip=0pt}
%       \caption{Experiment results on MATH dataset by subtopic. The setting of four prompting strategies are the are the same as Table \ref{table:math_main_results}.}
%       \label{fig:math_sub}
% \end{wrapfigure}
Table \ref{table:math_main_results} summarizes the performance of Self-Constructed  Prompting across 4 benchmarks in arithmetic reasoning. Overall, Self-Constructed  Prompting achieves competitive performance compared to either our experiments on Standard Prompting or published results. Since our prompting strategy reaches an comparable  score to Standard Prompting in both CoT and answer only scenario, we infer that it will significantly outperform zero-shot prompting, considering the significant performance gap between few-shot and zero-shot prompting mentioned in \citet{kojima2022large,brown2020language}. 

This results not only demonstrate the effectiveness and strong performance of Self-Constructed  Prompting, but also  question whether Standard Few-shot prompting truly enhance the model's capability on downstream tasks. Our experiments arguably demonstrate that for LLMs with the scale of  gpt-3.5-turbo, it inherently possesses the ability to achieve performance comparable to Few-shot prompting in both answer only and CoT. 



Surprisingly, we found that in GSM8K and MATH datasets, Self-Constructed CoT even outperform all other prompting strategies without any training datasets and human intervention. 
We speculate that the reason is that our few-shot examples and rationales are tailored to each test case, which might leading to better performance since it is more adaptive to individual cases. In contrast, Standard Prompting usually employ the same few-shot examples for an entire dataset instead of customizing for each individual case. 



Besides, with Self-Constructed CoT Prompting, gpt-3.5-turbo achives better performance compared to our baselines, outperforming Standard Prompting (33.5\% vs 31.2\% ). This suggests that Self-Constructed Prompting is still effective even when the task is highly demand for LLMs (with only a 33.5\% accuracy rate) .

Figure \ref{fig:math_sub} illustrates a detailed breakdown of the results for the MATH dataset, categorized by subtopics. We discovered Self-Constructed CoT outperforms Standard CoT in all 5 subtopics except Geometry. 
%error analysis
\subsection{Ablation Study}

==> table/app_detail_ablation.tex <==
\section{Details of Ablation Study}
\subsection{Details of Error Analysis in GSM8K}
\label{section:app_abla_gsm_err}
\paragraph{Correctness of Reasoning Process in Model-generated Few-shot Demonstrations} In almost all the examples we examined, the correctness of the reasoning process aligns with the correctness of the answers. We observed that in only two test samples (out of 40), the reasoning process was correct, but the answer and reasoning process did not match, which is incorrect. Additionally, there are cases where the answer is correct but the final extracted answer is incorrect due to insufficient accuracy in answer cleaning and extraction.
\paragraph{Error Type} We categorized the errors of the final predictions (not few-shot demonstrations) into three types: answer extraction errors, computation errors, and logical errors. In our 20 incorrect examples, only 1 sample belongs to answer extraction errors, 2 belong to computation errors, and the rest are logical errors, which are relatively more difficult to correct and identify.
% \subsection{Definition and Delineation of Errors of Few-shot Examples}
% \label{section:app_abla_def}
% The errors in the few-shot examples generated by LLM can be classified into four main categories: Answer extraction errors, Computation errors, Question errors and Logical errors. 
% \begin{itemize}
%     \item Answer extraction errors: This type of error occurs when the model's solution is correct, and the answer obtained from the solution is also correct. However, after going through answer cleaning and normalization, the answer is no longer correct. Please note that the cases where incorrect answers result from the integer normalization process are also considered answer extraction errors. That is why such errors still occur with a relatively high frequency even when we have a well-established answer extraction and normalization pipeline.
%     \item Computation errors: These errors occur during the reasoning process when the model performs calculations incorrectly, but the mathematical expressions or equations used in the process are correct.
%     \item Question errors: This type of error occurs when the question lacks necessary conditions, has ambiguity, or contains contradictions, resulting in an inability to answer.
%     \item Logical errors: Logical errors: Logical errors happen when the model follows an incorrect reasoning process, leading to an incorrect final answer. Generally, errors that do not fall into the first three categories are classified as logical errors.
% \end{itemize}

% We categorize Logical errors as fundamental errors, as they represent errors in the logical aspects of the model's reasoning. The other three types of errors are categorized as non-fundamental errors, as they don't involve errors at the logical level but rather concern shallower aspects like calculations, formatting, and so on.

\subsection{Definition and Delineation of Errors of Few-shot Examples}
\label{section:app_abla_def}
The errors in the few-shot examples generated by LLM can be classified into four main categories: Answer extraction errors, Computation errors, Question errors and Logical errors. 
\begin{itemize}
    \item Answer extraction errors: This type of error occurs when the model's solution is correct, and the answer obtained from the solution is also correct. However, after going through answer cleaning and normalization, the answer is no longer correct. Please note that the cases where incorrect answers result from the integer normalization process are also considered answer extraction errors. That is why such errors still occur with a relatively high frequency even when we have a well-established answer extraction and normalization pipeline.
    \item Computation errors: These errors occur during the reasoning process when the model performs calculations incorrectly, but the mathematical expressions or equations used in the process are correct.
    \item Question errors: This type of error occurs when the question lacks necessary conditions, has ambiguity, or contains contradictions, resulting in an inability to answer.
    \item Logical errors: Logical errors: Logical errors happen when the model follows an incorrect reasoning process, leading to an incorrect final answer. Generally, errors that do not fall into the first three categories are classified as logical errors.
\end{itemize}

We categorize Logical errors as fundamental errors, as they represent errors in the logical aspects of the model's reasoning. The other three types of errors are categorized as non-fundamental errors, as they don't involve errors at the logical level but rather concern shallower aspects like calculations, formatting, and so on.

\subsection{Why incorrect few-shot demonstrations could lead to correct results and correct few-shot demonstrations could lead to incorrect results?}
\label{section:app_abla_gsm_in_co}
We have thoroughly researched the detailed proportion of fundamental errors in few-shot examples that leading to correct results.
All but 4 cases of  the first row (where the final results of SEC are correct)  which belong to Major Error or All Incorrect  in Table \ref{table:abla_gsm_error} and Table \ref{table:app_err_gsm_diff} can be changed to Minor Error or All Correct by ignoring non-fundamental errors. Furthermore, among the remaining 4 samples, 2 of them are cases where the answer happens to be correct, meaning the reasoning process is incorrect, but it leads to the correct answer in the end. So, among the 40 correct samples we inspected, only 2 samples (5\%) that led to the correct final answer and reasoning had more than two few-shot demonstrations with a fundamentally flawed reasoning process and answer.

Section \ref{section:abla_mislead} mentioned several typical scenarios where incorrect few-shot demonstrations led to correct results. For these cases, we provide specific examples: answer extraction errors (see Figure \ref{fignl:cor_in_extraction}), computation errors (see Figure \ref{fignl:cor_in_cacu}), question errors (see Figure \ref{fignl:cor_in_ques}) and instances where the answer happened to be correct despite a flawed reasoning process (see Figure \ref{fignl:cor_in_happen}).

In addition, we also provide examples where correct few-shot demonstrations led to incorrect results. In most of these cases, the few-shot demonstrations were not sufficiently similar to the test question (see Figure \ref{fignl:in_cor_dissim}) or were too easy, leading the model to underestimate the difficulty of the final question (see Figure \ref{fignl:in_cor_easy}).


\subsection{Performance differences between  CoT-SEC and CoT-ICL in the GSM8K dataset}
\label{section:app_abla_gsm_diff}
In order to conduct a more in-depth study of the difference, following the manual inspection of correct and incorrect cases in the GSM8K dataset, we also randomly sampled 20 samples where  CoT-SEC was correct but  CoT-ICL was incorrect and 20 samples where CoT-SEC was incorrect but  CoT-ICL was correct. Then we further investigate the model-generated few-shot demonstrations of these 40 samples. The results are summarized in Table \ref{table:app_err_gsm_diff}.



\begin{table}[htbp]

    \begin{tabular}[]{p{2.8cm}p{1.9cm}| p{1.8cm}p{1.5cm}p{1.5cm}p{1.4cm}}
    \toprule
     CoT-SEC& CoT-ICL&  All Correct & Minor Error&Major Error & All Error\\
     \midrule
      Correct&Incorrect& 5/20&6/20  &6/20  &3/20  \\
      Incorrect&Correct& 2/20&5/20  &6/20  &7/20  \\
      
                       
    %  \\
    \bottomrule
\end{tabular}
\caption{Correctness of five few-shot demonstrations for 20 samples where  CoT-SEC was correct but CoT-ICL was incorrect, and 20 samples where CoT-SEC was incorrect but  CoT-ICL was correct in the GSM8K dataset. Minor Error means 1-2 incorrect examples, while Major Error means 3-4 incorrect examples.}
\label{table:app_err_gsm_diff}
\end{table}

It is reasonable that the quality of the generated few-shot demonstrations where CoT-SEC was correct but CoT-ICL was incorrect (shown in Table \ref{table:app_err_gsm_diff}) is lower than the average of samples where 
 CoT-SEC was correct (shown in Table \ref{table:abla_gsm_error}), since these examples are relatively more challenging for LLMs. And the quality of the generated few-shot demonstrations where CoT-SEC was incorrect but  CoT-ICL was correct (shown in Table \ref{table:app_err_gsm_diff}) is similar to where  CoT-SEC was incorrect (shown in Table \ref{table:abla_gsm_error}). 

We provided examples where CoT-SEC was correct but  CoT-ICL was incorrect (as shown in Figure \ref{fignl:cor_exam}), and examples where  CoT-SEC was incorrect but CoT-ICL was correct (as shown in Figure \ref{fignl:in_exam}). 



\subsection{Error analysis in HumanEval}
\label{section:app_abla_human}
% To further investigate the role and unique characteristics of model-generated few-shot examples, 
% we provided a comparison of the complexity between model-generated few-shot examples and canonical solutions. The complexity is measured by the length of the answer, i.e., the number of lines in the answer. The results are shown in Table \ref{table:app_err_human_comple}. It is evident that the complexity of the few-shot examples by the model is significantly smaller than the complexity of the canonical solutions, which leads to oversimplification in some test samples, especially the last three shots.

% \begin{table}[htbp]

%     \begin{tabular}[]{p{2cm}| p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{3cm}}
%     \toprule
%     &  $1^{st}$ shot & $2^{nd}$ shot&$3^{rd}$ shot&$4^{th}$ shot& Canonical Solution\\
%      \midrule
%       Avg. Lines& 7.3&6.9  &6.8  &7.1 &7.8   \\
      
                       
%     %  \\
%     \bottomrule
% \end{tabular}
% \caption{The average number of lines in model-generated examples and canonical solutions. The average length represents the complexity of the code to some extent.}
% \label{table:app_err_human_comple}
% \end{table}




To further investigate the role and unique characteristics of model-generated few-shot demonstrations, we conducted manual inspections on samples that exhibited changes in correctness (from correct to incorrect or incorrect to correct) when transitioning from k=1 to k=2 and from k=2 to k=3.  We examined these samples from four aspects:
\begin{enumerate}
    \item The correctness of model-generated few-shot demonstrations.
    \item The homogeneity of the model-generated few-shot demonstrations across different test samples.
    \item The type of error of the final output: Errors are categorized into two types: Logical Error and Grammar Error. Grammar Error only requires grammatical correction to become the correct answer, while Logical Error cannot be transformed into the correct answer with grammar correction alone.
    \item The complexity of the final output: Following the previous standard for measuring complexity, we adopt the number of lines in the answer.
\end{enumerate}
For detailed results of the error analysis, please refer to Table \ref{table:app_err_human_corr}, Table \ref{table:app_err_human_resul}.

From Table \ref{table:app_err_human_corr}, we could discover that the accuracy rate is quite high and approximately the same for each transition scenario. It shows that LLMs could produce few-shot demonstrations with high accuracy, and the correctness of the generated examples does not significantly impact the transition. Table \ref{table:app_err_human_resul} demonstrates that most of the errors of the final results in the transition  belong to Logical Error. 

\begin{table}[htbp]

    \begin{tabular}[]{p{3.1cm} p{2.1cm}|p{2.2cm}p{2.2cm}p{2.2cm}}
    \toprule
    \multicolumn{2}{c}{\textit{Transition}}  &\multicolumn{3}{c}{\textit{Accuracy of Model-generated demonstrations}}\\
    \cmidrule(r){1-2}
    \cmidrule(r){3-5}%
    Number of Shots&  Correctness &  $1^{st}$ shot&$2^{nd}$ shot &$3^{rd}$ shot \\
     \midrule
      1 shot $\rightarrow$ 2 shots &T $\rightarrow$ F &6/7  &7/7  &-    \\
      1 shot $\rightarrow$ 2 shots &F $\rightarrow$ T&11/13&10/13&-    \\
      2 shots $\rightarrow$ 3 shots&T $\rightarrow$ F &12/13&9/13 &11/13\\
      2 shots $\rightarrow$ 3 shots&F $\rightarrow$ T&3/3  &3/3  &3/3   \\
      
                       
    %  \\
    \bottomrule
\end{tabular}
\caption{The correctness of few-shot demonstrations generated by LLM in the HumanEval dataset where the correctness of the final output changes. Transition means the type of change these test samples experienced. For example, 1 shot $\rightarrow$ 2 shots and T $\rightarrow$ F means the final output of these examples is correct in 1 shot scenario while it is not correct in 2 shots scenario. The accuracy is represented in a/b, where a represents the number of correct cases, and b represents the total number of cases. Since in 1 shot $\rightarrow$ 2 shots scenario only the first two shots have an impact on the final correctness change,  we only examined the first two shots.}
\label{table:app_err_human_corr}
\end{table}



\begin{table}[htbp]

    \begin{tabular}[]{p{2.63cm} p{1.8cm}|p{2.5cm}p{2.5cm}|p{1cm} p{0.9cm}}
    \toprule
    \multicolumn{2}{c}{\textit{Transition}}   &\multicolumn{2}{c}{\textit{Error Type of the Incorrect Result}} &\multicolumn{2}{c}{\textit{Avg. Lines}}\\
    \cmidrule(r){1-2}
    \cmidrule(r){3-4}%
    \cmidrule(r){5-6}%
    Number of Shots&  Correctness & Logical Error & Grammar Error & Before &After\\
     \midrule
      1 shot $\rightarrow$ 2 shots &T $\rightarrow$ F   &6/7  &1/7 &\textcolor{red}{23.1}&\textcolor{red}{12.5}\\
      1 shot $\rightarrow$ 2 shots &F $\rightarrow$ T  &9/13 &4/13&15.4&14.1\\
      2 shots $\rightarrow$ 3 shots&T $\rightarrow$ F&12/13&1/13&12.8&13.0\\
      2 shots $\rightarrow$ 3 shots&F $\rightarrow$ T &3/3  &0/3 &9.7&9.7\\
      
                       
    %  \\
    \bottomrule
\end{tabular}
\caption{The  error type and length (measured by average lines)  of the final results in the HumanEval dataset where the correctness of the final output changes. The definition of transition is mentioned in the caption of Table \ref{table:app_err_human_corr}. The error type is also represented in a/b, where a represents the number of cases that belong to this particular error type, and b represents the total number of cases. In Avg. Lines, Before means before the transition while After means after the transition. For example, in 1 shot $\rightarrow$ 2 shots and T $\rightarrow$ F scenario, before means in 1 shot while after means in 2 shots.}
\label{table:app_err_human_resul}
\end{table}

\begin{wrapfigure}[11]{r}{0.4\textwidth}
    \vspace{-30pt}
    \begin{center}
      \includegraphics[width=0.4\textwidth]{asset/reverse_list_humaneval.pdf}
    \end{center}
    \captionsetup{skip=0pt}
    \caption{From 53.1\% (17 out of 32) of the test samples we examined, the question in the figure appears in the first two shots of the few-shot demonstrations generated.}
    \label{fig:reverse_list_humaneval}
\end{wrapfigure}



Based on the data from Table \ref{table:app_err_human_resul}, we can infer that during the transition from 1 shot to 2 shots, the reason for the change from correct to incorrect results might be that the complexity of the model-generated few-shot demonstrations are relatively low, leading the model to oversimplify the problem (avg. lines changes from 23.1 to 12.5). Then, we speculate that this trend of excessive simplification will continue to strengthen as the number of shots increases, although this change is not intuitively shown by the average line count. While the increase in performance with an increase in the number of shots is intuitive, this finding provides more insights into the reason that, after reaching a certain number of shots (1 or 2 shots), the performance actually decreases with an increase in shots.

Also, we made an astonishing additional discovery that  in the few-shot demonstrations generated from 53.1\% (17 out of 32) of the test samples we examined, the first two shots include one that is the same as the  question in Figure \ref{fig:reverse_list_humaneval}. This indicates that in the HumanEval dataset, the model-generated few-shot demonstrations are not as strongly related to the input questions as we initially anticipated. On the contrary, the few-shot demonstrations generated from different test samples are highly homogenized. This phenomenon is very different from what we observed in the GSM8K dataset. Also, the frequent occurrence of such simple questions  (in Figure \ref{fig:reverse_list_humaneval}) in model-generated few-shot examples further indicates that the model-generated demonstrations are too simplistic and underestimate the complexity of the problems.
\subsection{Performance of GSM8K on Different Models }
\label{section:app_abla_gsm_mode}
During the experiment on text-davinci-002 and text-davinci-003, we discover that  the model fails to generate  five demonstrations that all follow our output format. Frequently, the model only generates one demonstration, or it deviates from our output format starting from the second or third example. Therefore, we tentatively infer that these two models lack the capability to generate multiple good few-shot demonstrations, especially text-davinci-002. Thus, we only adopt 1 shot in these two models while adopting 5 shots in gpt-3.5-turbo.

\subsection{The similarity between few-shot examples and test question.} \label{section:abla_simi} We calculated the similarity between few-shot demonstrations  from  SEC and ICL, compared to the original questions. 
Our methodology involved utilizing the BERT model \citep{devlin-etal-2019-bert}  to procure embeddings for each set of example questions as well as the respective test questions. 
% To do this, we fed the question of both sets of examples  as well as the test question through BERT \citep{devlin-etal-2019-bert} to obtain their embeddings. 
Then we computed computed the cosine similarity between the embeddings to obtain the similarity score. Finally, We averaged the similarities of each shot to obtain the final similarity score of a particular prompting strategy.\footnote[4]{If the question used in vanilla ICL and CoT-ICL differ, we averaged the similarity scores from both prompting strategies to obtain the final similarity of ICL.} 
The results of all 6 datasets are shown in Figure \ref{fig:sim}. Also, we summarized the similarity of each shot in the GSM8K dataset in Figure \ref{fig:sim_gsm}.
{\setlength\intextsep{5pt}
\begin{figure}[h!]
    \centering
    \begin{minipage}{0.52\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{asset/similarity.pdf}
        \caption{The similarity between the few-shot demonstrations from SEC as well as ICL and the original questions of all 6 datasets.}
    \label{fig:sim}
    \end{minipage}
    \begin{minipage}{0.47\textwidth}
        \centering
        \includegraphics[width=0.97\linewidth]{asset/gsm_sim.pdf}
        \caption{The similarity of each shot in GSM8K dataset.}
    \label{fig:sim_gsm}
    \end{minipage}  
    
\end{figure}
}

The comparative analysis distinctly showcases a heightened similarity between the SEC and test questions, in contrast to ICL. This phenomenon further demonstrates the resemblance between SEC and $k$nn prompting\citep{xu2023k} which selected the few-shot examples based on $k$ Nearest Neighbors \citep{fix1989discriminatory}. Besides, Figure \ref{fig:sim_gsm} shows that in SEC, the similarity decreases as the index of the few-shot demonstrations increases. It is reasonable because as the index increases, they are further away from the test questions, making it harder for the model to reference them effectively. From the perspective of similarity, the quality of demonstrations decreases as the index increases.

\input{table/cor_in_extraction.tex}
\input{table/cor_in_cacu.tex}
\input{table/cor_in_ques.tex}
\input{table/cor_in_happen.tex}
\input{table/in_cor_dissimm.tex}
\input{table/in_cor_easy.tex}
\input{table/cor_exam.tex}
\input{table/in_exam.tex}

==> table/app_detail_exper.tex <==
\section{Details of Experimental SetUp}



\subsection{Tasks and datasets}
\label{section:app_det_task}
We tested our method on six datasets covering the fields of arithmetic reasoning, commonsense reasoning, and code generation.
A summary of our evaluation datasets is shown in Table \ref{tab:dataset}. 

\begin{table*}[!h]
   \small
   \centering
   \begin{tabular}{>{\centering\arraybackslash}p{4cm}|c|c|>{\centering\arraybackslash}p{4.7cm}|l}
   \toprule
   Dataset   & Split & Example & Domain                               & Metric \\
   \midrule
   GSM8K~\citep{cobbe2021training}       & Test   & 1319       & Arithmetic Reasoning             & acc   \\
   MATH~\citep{hendrycks2021measuring}   & Test   & 5000       & Arithmetic Reasoning                & acc\\
   AI2 Reasoning Challenge (ARC)~ \citep{clark2018think}& Test   & 1172  & Commonsense Reasoning      & acc \\
   MMLU~\citep{hendrycksmeasuring}       & Test   & 13985       & Multi-task Language Understanding                   & acc         \\
   C-Eval~\cite{huang2023c}              & Test   & 12342       & Multi-task Language Understanding in Chinese        & acc   \\
   HumanEval ~\cite{chen2021evaluating}  & Test   & 164       & Code Generation      & acc\\
   \bottomrule
   \end{tabular}
   \caption{A summary of our evaluation datasets. }
   \label{tab:dataset}
   \end{table*}

Here is a detailed description of datasets selection:

\textbf{Arithmetic Reasoning:} For arithmetic reasoning, we use GSM8K (grade-school math problems)
\citep{cobbe2021training} and MATH (high school level math competition problems) \citep{hendrycks2021measuring}.
Also, MMLU \citep{hendrycksmeasuring} and C-Eval \citep{huang2023c} contain mathematical questions. Therefore, we also provide 
the scores of these two datasets in their mathematics problem.

\textbf{Commonsense Reasoning:} Here we utilize AI2 Reasoning Challenge (ARC) \citep{clark2018think}, 
a grade-school level, multiple-choice science questions dataset.

\textbf{Multi-task Language Understanding:} For these tasks, we use MMLU (multi-choice questions in 57 domains)
 \citep{hendrycksmeasuring} and C-Eval (multi-choice questions across 52 diverse disciplines in China and four difficulty levels) 
 \citep{huang2023c}.    
 
\textbf{Code Generation:} We use HumanEval \citep{chen2021evaluating}, a collection of 164 hand-written programming problems.




\subsection{Models}\label{section:app_det_model} For our main results, we adopt ChatGPT (gpt-3.5-turbo)\footnote[5]{In our main experiments, 
we use gpt-3.5-turbo-0301 checkpoint, which will be deprecated later. However, we have discovered that gpt-3.5-turbo-0301 is highly likely to have undergone a model change on June 27th, the day OpenAI replaced the gpt-3.5-turbo checkpoint.
 },
%加入实验细节！
the most capable model in GPT-3.5 family\footnote[6]{https://platform.openai.com/docs/models/gpt-3-5}. And for some
ablation research, we also use text-davinci-003 and text-davinci-002 in GPT-3.5 family\footnote[7]{https://platform.openai.com/docs/models/gpt-3-5}. The key difference
between text-davinci-003 and text-davinci-002 is that text-davinci-003 was trained of HFRL, but text-davinci-002 was only trained with
supervised finetuning. 



\subsection{Details of Few-shot Extraction}
\label{section:app_det_extraction}
For more efficient extraction of few-shot demonstrations of the LLM output, we specify a desired output format in the prompt, as shown in Figure
\ref{fig:prompt}. Then, we parsed the output according to the format. 

In reality, the answer in the demonstration generated by LLMs may not always align with the answer format in the datasets. For example, LLMs might anser by the content of options rather than the option labels for a multi-choice question. Acknowledging these discrepancies, we perform answer extraction and answer validation for the generated answers to ensure that the answers are in the desired format. 
Initially, we follow the rules mentioned in Section \ref{section:result} to  extract and clean the answer for each few-shot demonstration. \footnote[3]{In the GSM8k dataset, it is a double-edged sword that normalizing all answers to integers to match the characteristics of the dataset's answers. Details in Appendix \ref{section:app_exp_det_nor}.} Then, each cleaned answer is validated to confirm its consistency with the predetermined format.
For all cases that did not pass the verification, we slightly alter the prompt  while setting the temperature to 1 to add
randomness. Then we have the LLM generate the demonstration again until it passes the validation.

\subsection{Prompts}
\label{section:app_det_prompt}
\subsubsection{The Source of Few-shot demonstrations in ICL}
\paragraph{Vanilla ICL} We used question answer pairs in the prompt in Minerva \citep{lewkowycz2022solving} for the MATH dataset, and the first five examples in the validation set for the ARC dataset. The few-shot demonstrations for MMLU and C-Eval datasets are  provided along the dataset. As for the HumanEval dataset, since there are no publicly available few-shot demonstrations and only a test set is provided, we select the first 4 test samples as the few-shot demonstrations for the remaining part of the test set, while choosing the last 4 test samples for the first 4 test samples.

\paragraph{CoT-ICL}We used the prompt in chain-of-thought Hub \citep{fu2023chain} for the GSM8K dataset, Minerva \citep{lewkowycz2022solving} for the MATH dataset. For the ARC dataset, we used the rationale generated by GPT4 model via ChatGPT official website\footnote[8]{https://chat.openai.com/?model=gpt-4     Using this feature requires subscribing to ChatGPT Plus.} for the first five examples in the validation set. The few-shot CoT prompts for MMLU and C-Eval datasets are  provided along the dataset. Since the HumanEval dataset directly prompts the model to generate a function body, it's weird to add CoT in a Python function. Thus we don't provide CoT results on HumanEval.


\subsubsection{Instruction for the Few-shot Demonstration Generation}
Table \ref{table:app_det_insr} summarizes the instruction used for the few-shot demonstration generation across all experiments.



\begin{table}[htbp]

    \begin{tabular}[]{p{2cm} | p{4.2cm}|p{6cm}}
    \toprule
    
    &Vanilla SEC &CoT-SEC \\
     \midrule
     MATH & Please follwing the above question, generate five similar questions with its answer in Latex.          &  Please follwing the above question, generate 5 similar questions with its step by step solution and answer in Latex.   \\
     \midrule
     GSM8K &Please generate five similar questions with integer answer&Please generate five similar questions with step by step reasoning process and an integer answer\\
     \midrule
     ARC &Follwing the above question, generate five similar multiple choice science questions with its choice labels, choice text and an answer label&Follwing the above question, generate ten similar multiple choice science questions with its choice labels, choice text, the explanation of the right answer and an answer label\\
     \midrule
     MMLU &Please follwing the above question, create five similar multiple choice \{\} questions with its choice labels, choice text and an answer label (A or B or C or D). Note that each question should be complete and can be answered independently.&Follwing the above question, generate five similar multiple choice \{\} questions with its choice labels, choice text, the step by step reason to choose your answer and an answer label (A or B or C or D). Note that each question should be complete and can be answered independently. \\
     \midrule
     C-Eval &
     \begin{CJK*}{UTF8}{gbsn}
        请模仿上面的问题，生成5个相似的关于\{\}考试的单项选择题，和这个这个题目的选项标签，选项内容和答案。每个问题必须是完整且能被独立回答的。
    \end{CJK*}&
    \begin{CJK*}{UTF8}{gbsn}
    请模仿上面的问题，生成5个相似的关于\{\}考试的单项选择题，和这个这个题目的选项标签，选项内容，逐步的推导出答案的过程和正确答案。每个问题必须是完整且能被独立回答的。
\end{CJK*}\\
     \midrule
     HumanEval &Following the example, generate 5 similar function headers with its function body in python.&-\\
                       
    %  \\
    \bottomrule
\end{tabular}
\caption{The instruction used for the few-shot demonstration generation across all 6 datasets. The \{\} in MMLU and C-Eval dataset will fill in specific subcategories.}
\label{table:app_det_insr}
\end{table}

\subsubsection{Output Format Instruction}
Table \ref{table:app_det_output} summarizes the instruction output format instruction across all experiments.
\begin{table}[htbp]

    \begin{tabular}[]{p{2cm} | p{4.45cm}|p{6.2cm}}
    \toprule
    
    &Vanilla SEC &CoT-SEC \\
     \midrule
     MATH & Please output in the following form [[Question1:{question}\textbackslash n Answer1:\$ answer in Latex\$ ]]\textbackslash n \textbackslash n  \textbackslash n \textbackslash n [[Question5:{question}\textbackslash n Answer5:\$ answer in Latex\$ ]]\textbackslash n \textbackslash n.&  Please output in the following form [[Question1:{question}\textbackslash n Sol1:[step by step solution]\textbackslash n Answer1:\$ answer in Latex\$ ]]\textbackslash n\textbackslash n \ldots  \textbackslash n\textbackslash n [[Question5:{question}\textbackslash n Sol5:[step by step solution]\textbackslash n Answer5:\$ answer in Latex\$ ]]\textbackslash n\textbackslash n.  \\
     \midrule
     GSM8K &in the following form Q1:\{ question\} \textbackslash n A1:\{ answer\} \textbackslash n \ldots  \textbackslash n Q5:\{ question\} \textbackslash n A5:\{ answer\} \textbackslash n.&in the following form Q1:\{ question\} \textbackslash n S1:\{ solution\} \textbackslash n A1:\{ answer\} \textbackslash n\textbackslash n \ldots  \textbackslash n\textbackslash n Q5:\{ question\} \textbackslash n S5:\{ solution\} \textbackslash n A5:\{ answer\} \textbackslash n\textbackslash n.\\
     \midrule
     ARC &in the following form [[Question1:\{ question\} \textbackslash n  Label1:[choice labels]\textbackslash n  Text1:[choice text]\textbackslash n  Ans1:\{ answer label\} ]]\textbackslash n \textbackslash n  \ldots \textbackslash n \textbackslash n  [[Question5:\{ question\} \textbackslash n  Label5:[choice labels]\textbackslash n  Text5:[choice text]\textbackslash n  Ans5:\{ answer label\} ]]\textbackslash n \textbackslash n .&in the following form [[Question1:\{ question\} \textbackslash n  Label1:[choice labels]\textbackslash n  Text1:[choice text]\textbackslash n  Sol1:\{ the explanation of the right answer\} \textbackslash n  Ans1:\{ answer label\} ]]\textbackslash n \textbackslash n  \ldots   \textbackslash n \textbackslash n  [[Question10:\{ question\} \textbackslash n  Label10:[choice labels]\textbackslash n  Text10:[choice text]\textbackslash n  Sol10:\{ the explanation of the right answer\} \textbackslash n  Ans10:\{ answer label\} ]]\textbackslash n \textbackslash n .\\
     \midrule
     MMLU &Please output in the following form [[Question1:[question]\textbackslash n  Label1:[choice labels]\textbackslash n  Text1:[choice text]\textbackslash n  Ans1:[A or B or C or D]]]\textbackslash n \textbackslash n  \ldots \textbackslash n \textbackslash n  [[Question5:[question]\textbackslash n  Label5:[choice labels]\textbackslash n  Text5:[choice text]\textbackslash n  Ans5:[A or B or C or D]]]\textbackslash n \textbackslash n .&Please output in the following form [[Question1:[question]\textbackslash n  Label1:[choice labels]\textbackslash n  Text1:[choice text]\textbackslash n  Sol1:[reason to choose your answer]\textbackslash n  Ans1:[A or B or C or D]]]\textbackslash n \textbackslash n \ldots  \textbackslash n \textbackslash n  [[Question5:[question]\textbackslash n  Label5:[choice labels]\textbackslash n  Text5:[choice text]\textbackslash n  Sol5:[reason to choose your answer]\textbackslash n  Ans5:[A or B or C or D]]]\textbackslash n \textbackslash n .\\
     \midrule
     C-Eval &    
     \begin{CJK*}{UTF8}{gbsn}
        请以以下格式输出答案：[[题目1:[题目]\textbackslash n  选项标签1:[选项标签]\textbackslash n  选项内容1:[选项内容]\textbackslash n  答案1:[A或B或C或D]]]\textbackslash n \textbackslash n  \ldots \textbackslash n \textbackslash n  [[题目5:[题目]\textbackslash n  选项标签5:[选项标签]\textbackslash n  选项内容5:[选项内容]\textbackslash n  答案5:[A或B或C或D]]]。
    \end{CJK*}
        &
        \begin{CJK*}{UTF8}{gbsn}
            请以以下格式输出答案：[[题目1:[题目]\textbackslash n  选项标签1:[选项标签]\textbackslash n  选项内容1:[选项内容]\textbackslash n  解析1：[逐步的推导出答案的过程]\textbackslash n  答案1:[A或B或C或D]]]\textbackslash n \textbackslash n  \ldots \textbackslash n \textbackslash n  [[题目5:[题目]\textbackslash n  选项标签5:[选项标签]\textbackslash n  选项内容5:[选项内容]\textbackslash n  解析5：[逐步的推导出答案的过程]\textbackslash n  答案5:[A或B或C或D]]]。
        \end{CJK*}\\
     \midrule
     HumanEval &Please output in the following form: [[[Function Header1]]:\textbackslash n  [[Function Body1]]: ]\textbackslash n \textbackslash n  \ldots \textbackslash n \textbackslash n  [[[Function Header5]]:\textbackslash n  [[Function Body5]]: ]\textbackslash n \textbackslash n .&-\\
                       
    %  \\
    \bottomrule
\end{tabular}
\caption{Output Format Instruction across all 6 datasets. The output format instruction contains numerous special symbols to facilitate better answer extraction, but these symbols may not be well presented in \LaTeX  ~formatting.}
\label{table:app_det_output}
\end{table}
\subsection{Unsimplified Illustration of SEC}
For better understanding, we have simplified SEC in Figure \ref{fig:prompt} of Section \ref{section:intro} and Figure \ref{fig:cot_prompt} of Appendix \ref{section:app_det_ill_cot}. We mainly simplified the output format in the few-shot demonstration generation, as the original format is designed for automatic recognition but might not be intuitive for understanding. Therefore, we transformed it into a more comprehensible format. The following Figure \ref{fig:fews_un} and Figure \ref{fig:cot_un} show the unsimplified illustration of Vanilla SEC and CoT-SEC.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{asset/few_un.pdf}
    \caption{The unsimplified illustration of Vanilla SEC.}
    \label{fig:fews_un}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{asset/cot_un.pdf}
    \caption{The unsimplified illustration of CoT-SEC}
    \label{fig:cot_un}
\end{figure}

\subsection{The detailed discussion on answer normalization in the GSM8k}
\label{section:app_exp_det_nor}
Not only might LLM's outputs fail to conform to the output format, but the questions generated by LLM may also not adhere to our instructions. This phenomenon is especially pronounced in the GSM8K dataset. The dataset's answers are represented as integers, but the questions generated by LLM may not always manipulate the data in a manner that results in an integer answer. Thus, We rounded the answers to integers so that they could meet the presentation format of the answer in the dataset.

However, the approach of directly rounding the answer may have negative effects on the performance of our method, despite the advantages mentioned above. Since the rounded answer is no longer the exact answer to the original question, there is a risk of misleading the model.  Despite the risks, we still decided to use it in the end, considering the advantages mentioned earlier and the convenience of normalization. The final experimental results were very satisfactory.
% 对于不符合指定的output format 的 case 的处理细节
\subsection{Details regarding the handling of cases that do not conform to the specified output format}
\label{section:app_det_not}
As mentioned earlier, in CoT-SEC, out of the 5000 samples in the MATH dataset, 6 samples were unable to generate few-shot demonstrations that conform to the specified output format. Meanwhile, in vanilla SEC, all 5000 samples generated few-shot demonstrations that meet the specified output format. Therefore, we decided to use the demonstrations in vanilla SEC on these 6 samples instead of CoT-SEC. Given that the overall performance of vanilla SEC is significantly lower than that of CoT-SEC, we believe that this approach is unlikely to overestimate the actual results of CoT-SEC. 
